Enable Deep Learning on Mobile Devices: Methods, Systems, and Applications

Deep neural networks (DNNs) have achieved unprecedented success in the field of artificial intelligence (AI), including computer vision, natural language processing and speech recognition. However, their superior performance comes at the considerable cost of computational complexity, which greatly hinders their applications in many resource-constrained devices, such as mobile phones and Internet of Things (IoT) devices. Therefore, methods and techniques that are able to lift the efficiency bottleneck while preserving the high accuracy of DNNs are in great demand in order to enable numerous edge AI applications. This paper provides an overview of efficient deep learning methods, systems and applications. We start from introducing popular model compression methods, including pruning, factorization, quantization as well as compact model design. To reduce the large design cost of these manual solutions, we discuss the AutoML framework for each of them, such as neural architecture search (NAS) and automated pruning and quantization. We then cover efficient on-device training to enable user customization based on the local data on mobile devices. Apart from general acceleration techniques, we also showcase several task-specific accelerations for point cloud, video and natural language processing by exploiting their spatial sparsity and temporal/token redundancy. Finally, to support all these algorithmic advancements, we introduce the efficient deep learning system design from both software and hardware perspectives.

==> algorithm/algo_sublinear_memory.tex <==
% \setlength{\textfloatsep}{0pt}
% \label{algo:sub_linear_training_memory_algo}
% \begin{algorithm}[!t]
% \footnotesize{
%     \SetAlgoLined
%     $v = input$ \\
%     \For{$k = 1 \mathbf{ \ to \ } length(segments)$}{
%         $temp[k] = v$ \\ 
%         \For{$i = segments[k].begin \mathbf{ \ to \ } segments[k].end - 1$}{
%             $v = layer[i].forward(v)$
%         }
%     }
%     $g = gradient(v, label)$ \\
%     \For{$k = length(segments) \mathbf{ \ to \ } 1$}{
%         $v = temp[k]$ \\
%         $localtemp = $ empty hashtable \\
%         \For{$i = segments[k].begin \mathbf{ \ to \ } segments[k].end - 1$}{
%             $localtemp[i] = v$ \\
%             $v = layer[i].forward(v)$ \\
%         }
%         \For{$i = segments[k].end - 1 \mathbf{ \ to \ } segments[k].begin$}{
%             $g = layer[i].backward(g, localtemp[i])$
%         }
%     }
%     \caption{Back-propagation with activation dropping \cite{chen2016training}.}
%     }
% \end{algorithm}


==> figText/fig_3d_applications_visualizations.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}[b]{0.49\textwidth}
    \centering
    % \includegraphics[width=\linewidth]{figures/applications/visualizations/1a}
    \includegraphics[width=\linewidth]{figures/3d_applications_2a}
    % \includegraphics[width=\linewidth]{figures/applications/visualizations/3a}
    \includegraphics[width=\linewidth]{figures/3d_applications_4a}
    %\includegraphics[width=\linewidth]{figures/3d_applications_5a}
    % \includegraphics[width=\linewidth]{figures/applications/visualizations/6a}
    % \includegraphics[width=\linewidth]{figures/applications/visualizations/7a}
    % \includegraphics[width=\linewidth]{figures/applications/visualizations/8a}
    \caption{MIT Driverless}
    \label{fig:applications:visualizations:a}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.49\textwidth}
    \centering
    % \includegraphics[width=\linewidth]{figures/applications/visualizations/1b}
    \includegraphics[width=\linewidth]{figures/3d_applications_2b}
    % \includegraphics[width=\linewidth]{figures/applications/visualizations/3b}
    \includegraphics[width=\linewidth]{figures/3d_applications_4b}
    %\includegraphics[width=\linewidth]{figures/3d_applications_5b}
    % \includegraphics[width=\linewidth]{figures/applications/visualizations/6b}
    % \includegraphics[width=\linewidth]{figures/applications/visualizations/7b}
    % \includegraphics[width=\linewidth]{figures/applications/visualizations/8b}
    \caption{PVCNN~\cite{liu2019point}}
    \label{fig:applications:visualizations:b}
\end{subfigure}
\caption{PVCNN~\cite{liu2019point} is much more accurate: \eg, MIT Driverless' model misclassifies the right traffic cone in the second example as blue. PVCNN also supports larger detection range, enabling the racing vehicle to confidently run at a higher speed.}
\label{fig:3d_applications:visualizations}
\end{figure*}

==> figText/fig_3d_constraint.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/3d_constraint.pdf}
    
    \caption{Overview for efficiency constraints in AutoML for point cloud understanding. Upper: LC-NAS~\cite{li2020lcnas} applies soft latency constraint at training time by adding a latency-related regularization term in the optimization objective. Lower: 3D-NAS~\cite{tang2020searching} applies hard efficiency constraint at search time such that all models exceeding the computation budget are directly rejected.}
    
    \label{fig:3d_constraint}
\end{figure}

==> figText/fig_3d_efficient_primitive.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/3d_primitive_sparseconv.pdf}
        \caption{Sparse Convolution~\cite{graham2015scn,graham2018sscn,choy20194d}}
        \label{fig:3d_efficient_primitives:sparseconv}
    \end{subfigure}
    %\hfill
    \begin{subfigure}{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/3d_primitive_pvconv.pdf}
        \caption{Point-Voxel Convolution~\cite{liu2019point}}
        \label{fig:3d_efficient_primitives:pvconv}
    \end{subfigure}
    \caption{Overview for representative efficient point cloud convolution modules. Sparse Convolution skips non-activated regions in both computation and storage and Point-Voxel Convolution eliminates irregular access and dynamic kernel computation cost of point-based methods.}
    \label{fig:3d_efficient_primitives}
\end{figure}


==> figText/fig_3d_spvnas.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}{0.485\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/3d_spvnas_1.pdf}
        \caption{Stage 1: Super Network Training.}
        \label{fig:3d_spvnas_stage1}
    \end{subfigure}
    %\hfill
    \begin{subfigure}{0.485\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/3d_spvnas_2.pdf}
        \caption{Stage 2: Evolutionary Architecture Search.}
        \label{fig:3d_spvnas_stage2}
    \end{subfigure}
    \caption{In the 3D-NAS~\cite{tang2020searching} framework, it first trains a super network composed of multiple SPVConvs, supporting fine-grained channel numbers and elastic network depths. Then, evolutionary architecture search is performed to obtain the best candidate model under a given computation constraint. \zhijian{Remove}}
    \label{fig:3d_spvnas}
\end{figure}





==> figText/fig_3d_teaser.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\columnwidth]{figures/3d_teaser.pdf}
    
    \caption{Efficient 3D deep learning is crucial in autonomous driving. The computation cost for 3D models is 28.5$\times$ higher than conventional image CNNs.}
    
    \label{fig:3d_teaser}
\end{figure}

==> figText/fig_nlp_fullstack.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.75\columnwidth]{figures/nlp_fullstack.pdf}
    
    \caption{Algorithm-hardware co-design across stack of several highlighted efficient NLP projects.}
    \label{fig:nlp_fullstack}
\end{figure}


==> figText/fig_nlp_hat_teaser.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\columnwidth]{figures/nlp_hat_teaser.pdf}
    
    \caption{Framework for searching Hardware-Aware Transformers. A SuperTransformer is firstly trained to contain numerous sub-networks, then evolutionary search with hardware latency feedback is performed to find one specialized SubTransformer for each hardware.~\cite{wang2020hat}}
    \label{fig:nlp_hat_teaser}
\end{figure}


==> figText/fig_nlp_spatten_teaser.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\columnwidth]{figures/nlp_spatten_teaser.pdf}
    \caption{Cascade token and head pruning removes redundant tokens and heads globally across layers.~\cite{wang2020spatten}}
    \label{fig:nlp_spatten_teaser}
\end{figure}


==> figText/fig_spatten_breakdown.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\columnwidth]{figures/perfbreak.pdf}
    
    \caption{Speedup Breakdown of SpAtten~\cite{wang2020spatten} over TITAN-Xp GPU on GPT-2 models. Cascade pruning and progressive quantization bring 3.4$\times$ and 2.8$\times$ speedup, respectively.}
    
    \label{fig:spatten_breakdown}
\end{figure}

==> figText/fig_topk.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.7\linewidth]{figures/topk.pdf}
\caption{High-parallelism top-k engine to rank token and head importance scores in SpAtten~\cite{wang2020spatten}.
}
\label{fig:topk}
\end{figure}

==> figText/hardware/enhcs/accuracy-vs-latency.tex <==
\begin{figure}[t]
\centering
    \includegraphics[width=0.33\linewidth]{figures/hardware/enhcs/ofa-edp.pdf}
    \hspace{10pt}
    \raisebox{5pt}{\includegraphics[width=0.38\linewidth]{figures/hardware/enhcs/arch.pdf}}
    \caption{Left: Accuracy \vs Normalized Energy-Delay-Product (EDP) on ImageNet (batch = 1). Co-searching architectural sizing with connectivity parameters and mapping strategy outperforms searching architectural sizing alone (NHAS~\cite{linneural}). Integrating with OFA NAS further improves model accuracy. Right: Searched hardware design for 78\% accuracy point is a X'-K paralleled architecture with array size of 18$\times$10, which differs from common architectures' parallelism: X-Y (ShiDianNao), C-K (EdgeTPU, NVDLA), R-Y' (Eyeriss).~\cite{lin2021enhcs}}
    \label{fig:hardware_enhcs_qnas-res}
\end{figure}


==> figText/hardware/enhcs/modeling.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/hardware/enhcs/modeling.pdf}
    \caption{NAAS~\cite{lin2021enhcs} encodes the hardware design and compiler mapping strategy into vectors. A hardware design is described by architectural sizing and connectivity parameters, where PE inter-connection is presented by parallel dimension. A mapping strategy is represented by loop order and corresponding tiling at each dimension of array (the innermost level is PE level).}
    \label{fig:hardware_enhcs_modeling}
\end{figure*}

==> figText/hardware/enhcs/no_ordering.tex <==
\begin{figure}[t]
\centering
    \includegraphics[width=0.45\linewidth]{figures/hardware/naas/no-ordering.pdf}
    \caption{Compared to searching the architectural sizing only~\cite{yang2020co, linneural}, searching the connectivities and mappings as well (NAAS~\cite{lin2021enhcs}) achieves considerable EDP reduction.}
    \label{fig:hardware_enhcs_no-ordering}
\end{figure}


==> figText/hardware/enhcs/ordering.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/hardware/enhcs/ordering.pdf}
    \caption{NAAS converts the non-numerical ordering optimization into numerical optimization. When generating a possible hardware/mapping candidate, the encoding vector assigns each loop dimension with an importance value. These importance values are sorted to obtain the corresponding order. In the example, since array \#dim is 2, the first two sorted dimension is chosen and thus hardware is designed to parallelize the computation at dimension K and C.~\cite{lin2021enhcs}}
    \label{fig:hardware_enhcs_ordering}
\end{figure}

==> figText/hardware/fig_dataflow.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/hardware/weight_stationary.pdf}
    \includegraphics[width=\columnwidth]{figures/hardware/output_stationary.pdf}
    \includegraphics[width=\columnwidth]{figures/hardware/no_local_reuse.pdf}
    \caption{DNN Accelearator Dataflows~\cite{sze2017efficient}: (a) Weight Stationary; (b) Output Stationary; (c) No Local Reuse}
    \label{fig:hardware_dataflow}
\end{figure}

==> figText/hardware/fig_enhas.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\linewidth]{figures/hardware/enhcs/naas.pdf}
    \caption{Neural Accelerator Architecture Search (NAAS) using evolution algorithms~\cite{linneural}.}
    \label{fig:naas}
\end{figure}

==> figText/hardware/fig_enhas_results.tex <==
\begin{figure}[t]
\centering
    \includegraphics[width=0.55\linewidth]{figures/hardware/qnas-res.pdf}
    \caption{Improvement Breakdown from Each Optimization Step: Baseline $\rightarrow$ EHAS only $\rightarrow$ EHAS+QNAS $\rightarrow$ ENHAS in One Loop. (Accuracy \vs Latency on ImageNet, batch = 1)~\cite{linneural}.}
    \label{fig:hardware_enhas_res}
\end{figure}

==> figText/hardware/fig_has_grid.tex <==
\begin{figure}[t]
\centering
    \includegraphics[width=0.55\linewidth]{figures/hardware/has-bitfusion-vs-grid-arrow-results.pdf}
    \caption{EHAS in ENHAS~\cite{linneural} is able to find solutions with better trade-off between area budget and energy-delay product.}
    \label{fig:hardware_has_grid}
\end{figure}

==> figText/hardware/fig_parallel.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/hardware/parallel_compute.pdf}
    \caption{Highly parallel compute paradigms~\cite{sze2017efficient}}
    \label{fig:hardware_parallel}
\end{figure}

==> figText/hardware/sparch/fig_4steps.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\columnwidth]{figures/hardware/sparch/tp_4steps.pdf}
    \caption{Performance of SpArch~\cite{sparch} in comparisons with OuterSPACE~\cite{pal2018outerspace}. The first slowdown is because of the excessive memory access of partially merged results when the number of partial matrices is much larger than merge tree parallelism. But it enables the next three optimizations.
    % We save DRAM bandwidth, achieve higher memory utilization and speedup.
    }
    \label{fig:hardware_sparch_tp_4steps}
\end{figure}

==> figText/hardware/sparch/fig_huffman.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/hardware/sparch/tp_huffman.pdf}
    \caption{Huffman tree scheduler in SpArch~\cite{sparch} gives near optimal order of partial matrices merging. The total memory access is minimized. The weights of nodes represent the number of non-zeros in the partial matrices.  The total DRAM access is proportional to the sum of nodes' weights.}
    \label{fig:tp_huff}
\end{figure}

==> figText/hardware/sparch/fig_teaser.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\columnwidth]{figures/hardware/sparch/teaser.pdf}
    \caption{Outer product based SpGEMM architecture SpArch~\cite{sparch} jointly optimizes input and output data reuse. It achieves good output reuse with pipelined multiply and merge, matrix condensing, Huffman tree scheduler, and good input reuse with a row prefetcher. }
    \label{fig:hardware_sparch_teaser}
\end{figure}

==> figText/tab_3d_applications_results.tex <==
\begin{table}[!t]
\setlength{\tabcolsep}{10pt}
\small\centering
\begin{tabular}{lccc}
    \toprule
    & Detection Range (m) & GPU Latency (ms) & Accuracy (\%) \\
    \midrule
    MIT Driverless & 8 & 14 & 95 \\
    PointNet~\cite{qi2017pointnet} & \textbf{12} & 31.5 & 97 \\
    \midrule
    \textbf{PVCNN}~\cite{liu2019point} & \textbf{12} & \textbf{8.75} & \textbf{99.93} \\
    \bottomrule
\end{tabular}
\caption{Results of traffic cone classification for autonomous racing vehicle: compared with MIT Driverless' model, PVCNN~\cite{liu2019point} achieves larger detection range, higher accuracy and lower latency. Here, we measure the GPU latency based on an average of 7 cones per scene.}
\label{tab:3d_applications:results}
\end{table}
